Measurement of the inclusive isolated prompt photon cross section in pp collisions at sqrt(s) = 7 TeV with the ATLAS detector using 4.6 fb-1

A measurement of the cross section for the production of isolated prompt photons in pp collisions at a center-of-mass energy sqrt(s) = 7 TeV is presented. The results are based on an integrated luminosity of 4.6 fb-1 collected with the ATLAS detector at the LHC. The cross section is measured as a function of photon pseudorapidity and transverse energy in the kinematic range between 100 GeV and 1000 GeV and in the regions of pseudorapidity less than 1.37 and between 1.52 and 2.37. The results are compared to leading-order parton-shower Monte Carlo models and next-to-leading-order perturbative QCD calculations. Next-to-leading-order perturbative QCD calculations agree well with the measured cross sections as a function of transverse energy and pseudorapidity.

==> systematics.tex <==
The integrated luminosities are calculated during runs by measuring
interaction rates using several ATLAS devices at small angles to the
beam direction, with the absolute calibration obtained from Van der
Meer scans. 
The relative systematic uncertainty on the luminosity measurement is
estimated to be $1.8\%$
\cite{ATLAS-CONF-2011-011} 
and translates directly into a $1.8\%$ relative uncertainty on the cross-section. 
This uncertainty, which scales every point of the differential cross sections either up or down,
is not added in quadrature to other uncertainties and thus should be considered separately.



 
 

